RETAIN: Interactive Tool for Regression Testing Guided LLM Migration

Large Language Models (LLMs) are increasingly integrated into diverse applications. The rapid evolution of LLMs presents opportunities for developers to enhance applications continuously. However, this constant adaptation can also lead to performance regressions during model migrations. While several interactive tools have been proposed to streamline the complexity of prompt engineering, few address the specific requirements of regression testing for LLM Migrations. To bridge this gap, we introduce RETAIN (REgression Testing guided LLM migrAtIoN), a tool designed explicitly for regression testing in LLM Migrations. RETAIN comprises two key components: an interactive interface tailored to regression testing needs during LLM migrations, and an error discovery module that facilitates understanding of differences in model behaviors. The error discovery module generates textual descriptions of various errors or differences between model outputs, providing actionable insights for prompt refinement. Our automatic evaluation and empirical user studies demonstrate that RETAIN, when compared to manual evaluation, enabled participants to identify twice as many errors, facilitated experimentation with 75% more prompts, and achieves 12% higher metric scores in a given time frame.

==> sections/7_Limitations.tex <==
\section{Limitations}
\label{limitations}
%In addition to the above features, through our user study we discovered opportunities to further enhance users’ analysis. \modelname doesn't support creation of metrics on the fly. Practitioners would like to create rule based metrics on the fly to deterministically catch certain error types. This can be easily implemented with regex based filtering. \modelname doesn't provide prompt edit suggestions, with the rise of automatic prompt engineering techniques \cite{khattab2023dspy}, including prompt edit suggestions could facilitate faster prompt migrations. 

Our user study revealed several opportunities to further enhance \modelname's analytical capabilities:
\begin{itemize}
    \item On-the-Fly Metric Creation: Users expressed a desire to create rule-based metrics during analysis to deterministically catch specific error types. This could be implemented using regex-based filtering, allowing for more flexible and immediate error detection.
    \item Prompt Edit Suggestions: Currently, \modelname doesn't provide automated prompt edit suggestions. Incorporating automatic prompt engineering techniques, as demonstrated by \citet{khattab2023dspy}, could significantly accelerate the prompt migration process.
\end{itemize}
These potential enhancements aim to increase \modelname's flexibility and efficiency, further streamlining the prompt engineering workflow for LLM developers and researchers. 
\\ \\
In addition, it's important to note a key limitation in our evaluation: We did not formally assess the efficacy of \modelname on long document scenarios, focusing primarily on short to mid-size text. This limitation largely stems from the immense complexity inherent in long-document fine-tuning scenarios and was primarily a restriction of time in our studies. As LLMs are increasingly used for processing and generating longer documents, future work should extend the evaluation to include these more complex, lengthy scenarios. This would ensure \modelname's effectiveness across a broader range of text lengths and complexities, despite the additional challenges posed by long-document analysis.
